Automating Sized Type Inference for Complexity Analysis (Technical Report)

This paper introduces a new methodology for the complexity analysis of higher-order functional programs, which is based on three ingredients: a powerful type system for size analysis and a sound type inference procedure for it, a ticking monadic transformation, and constraint solving. Noticeably, the presented methodology can be fully automated, and is able to analyse a series of examples which cannot be handled by most competitor methodologies. This is possible due to the choice of adopting an abstract index language and index polymorphism at higher ranks. A prototype implementation is available.

==> implementation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Specialising Types to Call-sites.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  Higher-order combinators such $\fun{map}$, $\fun{filter}$ or the various fold combinators
  allow concise but readable definitions. Consequently, their use is pervasive in functional programming
  and has to be addressed in a practical system.
  Consider for instance the combinator $\fun{foldr}$:
  \begin{alignat*}{2}
    & \mparbox{0mm}{\fun{foldr} \decl \forall \tyvarone \tyvartwo.\ (\tyvarone \starr \tyvartwo \starr \tyvartwo) \starr \tyvartwo \starr \tylist[]{\tyvarone} \starr \tyvartwo}\\
    & \fun{foldr} \api f \api b \api \con{Nil} && = b \\ 
    &\fun{foldr} \api f \api b \api (\con{Cons} \api x \api xs) && = 
    f \api x \api (\fun{foldr} \api f  \api b \api xs)
      \tpkt
    \end{alignat*}
    This combinator allows us to concisely define the concatenation of lists by
  \begin{align*}
    & \fun{concat} \decl \forall \tyvarone.\ \tylist{\tylist{\tyvarone}} \starr \tylist{\tyvarone}\\
    & \fun{concat} = \fun{foldr} \api (\fappend) \api \con{Nil} \tkom
  \end{align*}
  where $(\fappend)$ denotes the append functions defined in the usual way.
  In the system that we have seen so far, it is not difficult to infer
  \[
    (\fappend) \decl \forall \tyvarone.\ \forall \ivarone\ivartwo.\ \tylist[\ivarone]{\tyvarone} \starr \tylist[\ivartwo]{\tyvarone} \starr \tylist[(\ivarone - 1) + \ivartwo]{\tyvarone}
    \tpkt
  \]  
  %
  However, using only an annotation of the principal type of $\fun{foldr}$ as above, 
  the typing of the body of $\fun{concat}$ would require that the call to $(\fappend)$ is 
  typed as an instance of $\tyvarone \starr \tyvartwo \starr \tyvartwo$. This again is only possible when 
  $(\fappend)$ is given the type $\tylist[1]{\tyvarone} \starr \tylist[c]{\tyvarone} \starr \tylist[c]{\tyvarone}$, 
  and consequently, $\fun{concat}$ will be given a type
  \[
    \forall \ivarthree.\ \tylist[\ivarthree]{(\tylist[1]{\tyvarone})} \starr \tylist[c]{\tyvarone} \tkom
  \]
  for some (arbitrary) expression $c$.
  Although such a type is legitimate, it is of limited use. The function can then only be applied to concatenate empty lists.

  The way out is to specialise types of higher-order combinators, such as $\fun{foldr}$, suitable to specific uses of the combinator. 
  E.g., we would specialise the type of fold to 
  \[
    \forall \tyvarone\tyvartwo.\ (\tylist{\tyvarone} \starr \tylist{\tyvartwo} \starr \tylist{\tyvartwo}) \starr \tylist{\tyvartwo} \starr \tylist[]{(\tylist{\tyvarone})} \starr \tylist{\tyvartwo}
    \tkom
  \]
  which can then be given more concrete size annotations.
  Specialisation, together with the feature discussed next, will allow us to check 
  \[
    \fun{concat} \decl \forall \ivarone\ivartwo.\ \tylist[\ivarone]{(\tylist[\ivartwo]{\tyvarone})} \starr \tylist[(\ivarone -1)\cdot(\ivartwo -1) + 1]{\tyvarone} \tpkt
  \]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

